Telechain: Bridging Telecom Policy and Blockchain Practice

The use of blockchain in regulatory ecosystems is a promising approach to address challenges of compliance among mutually untrusted entities. In this work, we consider applications of blockchain technologies in telecom regulations. In particular, we address growing concerns around Unsolicited Commercial Communication (UCC aka. spam) sent through text messages (SMS) and phone calls in India. Despite several regulatory measures taken to curb the menace of spam it continues to be a nuisance to subscribers while posing challenges to telecom operators and regulators alike. In this paper, we present a consortium blockchain based architecture to address the problem of UCC in India. Our solution improves subscriber experiences, improves the efficiency of regulatory processes while also positively impacting all stakeholders in the telecom ecosystem. Unlike previous approaches to the problem of UCC, which are all ex-post, our approach to adherence to the regulations is ex-ante. The proposal described in this paper is a primary contributor to the revision of regulations concerning UCC and spam by the Telecom Regulatory Authority of India (TRAI). The new regulations published in July 2018 were first of a kind in the world and amended the 2010 Telecom Commercial Communication Customer Preference Regulation (TCCCPR), through mandating the use of a blockchain/distributed ledgers in addressing the UCC problem. In this paper, we provide a holistic account of of the projects' evolution from (1) its design and strategy, to (2) regulatory and policy action, (3) country wide implementation and deployment, and (4) evaluation and impact of the work.

==> sections/appendices.tex <==
\appendix

\section{History of Regulatory Amendments to UCC in India}

Since the effect of the Telecom Commercial Communications Customer Preference Regulations (TCCCPR) in 2010, TRAI in the 6\textsuperscript{th} amendment introduced a SMS header format (AB-XXXXXX) where \textit{AB} corresponds to the telecom provider and region and \textit{XXXXXX} corresponds to the alpha numeric code for the business entity sending the promotional SMS. The amendment to the regulation clearly defined \textit{promotional} \& \textit{transactional} messages in addition to demarcating special phone number sequences which begin with \textit{+91-140} for telemarketers to use during promotional phone calls~\cite{traireg2010}. A \textit{promotional} SMS is used to send offers, discounts or promotions to new or existing customers which may have not been solicited by the recipients and can only be sent between 9AM and 9PM. A \textit{transactional} SMS is used to send one time passwords, informational messages, booking information or order alerts to registered customers and should not be intended for marketing.


The 2010 regulatory mandate also involved an online registration process for telemarketers starting 15th January 2011 by paying 1000 INR (approx. 13.5 USD), and 9000 INR (approx. 120 USD) as customer education fee. Once validated, the telemarketers are immediately assigned a telemarketer ID, and issued a registration certificate for beginning operations~\cite{traitelemarketerregistration}. Malicious telemarketers found ways to register small fraudulent entities and paid the low registration cost of 10000 INR (approx. 133.5 USD) to access and obtain numbers from the national registry. The malicious telemarketers then use personal phone numbers to send promotional SMS content mimicking the standard peer to peer (P2P) messages which are treated differently than business messages (Note that business messages or bulk ads are 8 times more expensive than P2P SMS). These operations are extremely hard to detect without privacy invasive checks on all customer communications and the telecom operators therefore resort to reactive approaches such as investigation procedures when affected subscribers file complaints with the operator or with the regulatory body. These telemarketers are classified as unregistered telemarketers. In response to increasing cases of fraud and telemarketing from unregistered telemarketers, TRAI capped the number of SMSs that can be sent in a day to 100 per day and limited to 3000 per month for mobile subscribers which was later amended to 200 per day. In the 10\textsuperscript{th} amendment of the regulation, TRAI mandated the usage of \textit{signature solutions} by telecom operators to detect bulk messages having similar string or their variants, specifically those without any specific information of the subscriber. Additional improvements in the amendment included guidelines for block-listing or throttling specific numbers, introducing higher tariffs for bulk messaging, and a web based complaint registration system. In the 13\textsuperscript{th} amendment, the regulation introduced financial disincentives to telecom operators and telemarketers for complaints registered about violations of users' preferences and increased the security deposit needed to be made by the telemarketers to be registered. A recent summary by Tu \textit{et al.} identifies the various techniques currently in use to curb UCC due to robocalls in the United States and similar systems implemented and adopted across the world by various telecom operators~\cite{sokrobocalls}.

Despite incessant measures taken to mandate the use of the NDND registry and regulating the usage of specific number series and SMS header, customer dis-satisfaction continued, indicating the increasing challenges faced by the ecosystem, hinting towards the possible need for revising the regulatory framework.



% \section{Questions to ask}

% \begin{enumerate}
% 	\item What is the number of people registered on the TRAI DND database? % 230 million (https://www.capacitymedia.com/articles/3811786/India-to-enforce-national-blockchain-database-for-do-not-call-register)
% 	\item What is the total number of complaints that have been registered since the inception of the DND Registry?
% 	% 2 million complaints, 40K per month P59 (https://main.trai.gov.in/sites/default/files/RegulationUcc19072018.pdf)
% 	\item How many complaints are registered via the TRAI mobile applications and from the telecom companies (daily / weekly / monthly granularity)? [This might be a good graph to have] {Yearwise is available in the updated regulation and consultation documents}
% 	\item What is the total number of registered telemarketers? % 7986 (http://www.nccptrai.gov.in/nccpregistry/ListofTelemarketers.do?method=getTMRegList&EIID=&districtcode=&statecode=1)
% 	\item How many of the registered telemarketers have been banned, fined in the past few years?
% 	\item What is the total volume of promotional and transactions SMSs that flow in India to subscribers daily/weekly/monthly?
% 	\item Are there any existing consent capturing and maintenance procedures in place?
% 	\item What is the average time taken to take action on a UTM by a telecom? How many such actions were taken?
% 	\item What is the time taken currently for a DND / Preference registration to be reflected on all the Telecom operators databases? (7 days from what I last remember) [There's quite some content provided in the \textit{Analysis of present system} of the regulation].
% 	\item What is the economic value of telemarketing in India using SMS and Voice?
% 	\item What are the total number of SMS/Calls for telemarketing \& promotions made on a daily basis in India?
% 	\item How many subscribers are currently registered on the DND registry?
% 	\item How has the introduction of DND registry changed the way in which people experienced UCC before its introduction? What were the limitations?
% 	\item How many registered telemarketers are in tier 2 and tier 3 towns and villages in the country? What is their yearly volume of SMS \& call based marketing? Is there a category wise breakdown of marketing which is done by these telemarketers?
% 	\item What is the average size of a promotional campaign list that is used by the telemarketers for scrubbing?
% \end{enumerate}



==> sections/findings.tex <==
\section{Research Context}

\subsection{Organizational}
\subsection{Cost}
\subsection{Regulation}
\subsection{Privacy}

==> sections/introduction.tex <==
\section{Introduction}
This is the Introduction Section.
